Why Software Signing (Still) Matters: Trust Boundaries in the Software Supply Chain

Software signing provides a formal mechanism for provenance by ensuring artifact integrity and verifying producer identity. It also imposes tooling and operational costs to implement in practice. In an era of centralized registries such as PyPI, npm, Maven Central, and Hugging Face, it is reasonable to ask whether hardening registry security controls obviates the need for end-to-end artifact signing. In this work, we posit that the core guarantees of signing, provenance, integrity, and accountability are not automatically carried across different software distribution boundaries. These boundaries include mirrors, corporate proxies, re-hosting, and air-gapped transfers, where registry security controls alone cannot provide sufficient assurance. We synthesize historical practice and present a trust model for modern distribution modes to identify when signing is necessary to extend trust beyond registry control. Treating signing as a baseline layer of defense strengthens software supply chain assurance even when registries are secure.

==> misc/typesetting-old.tex <==
% Pre-condition: Set the ifs: \ifDEBUG, \ifANONYMOUS, \ifSPACEHACK

%%%%%
% Standard packages
%%%%%


%\usepackage[compress]{cite} % numbered ordering of multiple citations, set to compress ranges
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{booktabs} % For formal tables \toprule
\usepackage{xspace} % Put an \xspace within numeric macros
\usepackage[normalem]{ulem}
\usepackage{makecell}
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage[vskip=1em,font=itshape,leftmargin=2em,rightmargin=2em]{quoting}
\usepackage{svg}
\usepackage{listings}
\usepackage{subfigure}
\usepackage{xcolor}
\usepackage{url}
\def\UrlBreaks{\do\/\do-\do_} % Defining where it is okay to wrap a url to a new line. For bibliography.
%\useunder{\uline}{\ul}{}
% \usepackage{filecontents,lipsum}
% \usepackage[noadjust]{cite}
%%%%%
% Comments and TODOs
%%%%%

\usepackage{soul}
\usepackage{hyperref}
\usepackage{cleveref}

\ifDEBUG
    % Floating comment boxes
    \newcommand{\JD}[1]{\textcolor{blue}{[Jamie: #1]}}
    \newcommand{\Kelechi}[1]{\textcolor{olive}{[Kelechi: #1]}}
    \newcommand{\TRS}[1]{\textcolor{orange}{[Taylor: #1]}}
    \newcommand{\AK}[1]{\textcolor{purple}{[Andy: #1]}}
    \newcommand{\ST}[1]{\textcolor{red}{[Santiago: #1]}}
    \newcommand{\SB}[1]{\textcolor{red}{[Saurabh: #1]}}
    \newcommand{\Eman}[1]{\textcolor{teal}{[Eman: #1]}}
    % Inline comments and WIP phrasing
    \newcommand{\TODO}[1]{\hl{#1}}
    \newcommand{\CHOP}[1]{}
    \newcommand{\placeholder}[1]{\hl{#1}}


    \hypersetup{
        pdfpagemode=UseNone % don't show thumbnails or bookmarks on opening
    }

\else
    \newcommand{\JD}[1]{}
    \newcommand{\Kelechi}[1]{}
    \newcommand{\TRS}[1]{}
    \newcommand{\AK}[1]{}
    \newcommand{\ST}[1]{}
    \newcommand{\SB}[1]{}
    \newcommand{\Eman}[1]{}
    \newcommand{\TODO}[1]{}
    \newcommand{\CHOP}[1]{}
    \newcommand{\placeholder}[1]{#1}
\fi

%%%%%
% Paragraph-level labels
%%%%%

%%%%%
% Space hacking
%%%%%

% To reduce spacing after headings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{titlesec}

% \usepackage[compact]{titlesec}
% \titleformat{\section}
%   {\normalfont\Large\bfseries}{\thesection}{1em}{\MakeUppercase}
%     % The bug in the new version 2.10.1 is not properly starting horizontal mode
%     % http://tex.stackexchange.com/questions/299969/titlesec-loss-of-section-numbering-with-the-new-update-2016-03-15
%     \usepackage{etoolbox}
%     \makeatletter
%     \patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
%     \patchcmd{\ttlh@hang}{\noindent}{}{}{}
%     \makeatother

% Make a \paragraph that is inline and emphasized
\newcommand{\myparagraph}[1]{\vspace{0.08cm}\noindent\hspace{0.1cm} \textit{#1:}}

\newcommand{\myminisection}[1]{\vspace{0.1cm} \noindent \textbf{#1.}}

\newcommand{\mysubsubsection}[1]{\subsubsection{\textbf{#1}}}

% \ifSPACEHACK
%     % Titlespacing args: \titlespacing{command}{left spacing}{before spacing}{after spacing}[right]
%     \titlespacing*\subsection{0pt}{2pt plus 1.5pt minus 1.5pt}{1pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\subsubsection{0pt}{2pt plus 1pt minus 1pt}{2pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\paragraph{0pt}{2.5pt plus 1.5pt minus 1.5pt}{2pt plus 1.5pt minus 1.5pt}
%     \setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\floatsep}{2.0pt plus 2.0pt minus 2.0pt}
%     %\setlength{\textfloatsep}{3.0pt plus 2.0pt minus 4.0pt}
%     %\setlength{\intextsep}{2.0pt plus 2.0pt minus 2.0pt}
% \fi

%%%%%%%%
% Peer review
%%%%%%%%


%%%%%%%%
% Balance references
%%%%%%%%

\usepackage{balance} % Put \balance on the last page
%\usepackage{caption}
%\usepackage[font=normal]{caption}
% \usepackage{subcaption}
%%%%
% Intra-paper references
%%%%

\usepackage{amsmath}
\usepackage{cleveref}


\crefformat{section}{\S#2#1#3}
\crefrangeformat{section}{\S#3#1#4--\S#5#2#6}
\crefname{figure}{Figure}{Figures}
\crefname{appendix}{Appendix}{Appendices}
\crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{listing}{Listing}{Listings}
\crefname{theorem}{Theorem}{Theorems}
\crefname{thm}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{equation}{Eqt.}{Eqts.}
\crefformat{Grammar}{Grammar #1}


%%%%
% Tunable enumerate and itemize
%%%%

\usepackage{enumitem}
\usepackage{booktabs}

%%%%
% Latin
%%%%

\newcommand{\ie}{\textit{i.e.,} }
\newcommand{\eg}{\textit{e.g.,} }
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\nb}{\textit{N.B.,} }

\newcommand{\HF}{{Hugging Face}\xspace}
% Please add the following required packages to your document preamble:

\usepackage{enumitem}

%\usepackage{booktabs}
%\usepackage[normalem]{ulem}

% Nice formatting for a list of RQs
\newenvironment{RQList}{
   \setlength{\topsep}{0pt}
   \setlength{\partopsep}{0pt}
   \setlength{\parskip}{0pt}
   \begin{description}[style=unboxed]
   \setlength{\leftmargin}{1in}
   \setlength{\parsep}{0pt}
   \setlength{\parskip}{0pt}
   \setlength{\itemsep}{0pt}
   }
   {\end{description}}
   
\setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
\setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}

\newcommand{\myquote}[1]{\begin{quote}\emph{``#1''}\end{quote}}
\newcommand{\myinlinequote}[1]{\emph{``#1''}}

\newcommand{\SmallLongString}[1]{ {\small \emph{#1}}\xspace}

% ParticipantID, Quote
\newcommand{\ParticipantQuote}[2]{
    \begin{quote}
    \emph{\textbf{#1}: ``#2''} 
    \end{quote}}
    
\DeclareUnicodeCharacter{2060}{\nolinebreak}

